Nonparametric homogeneity tests and multiple change-point estimation for analyzing large Hi-C data matrices

We propose a novel nonparametric approach for estimating the location of block boundaries (change-points) of non-overlapping blocks in a random symmetric matrix which consists of random variables having their distribution changing from one block to the other. Our method is based on a nonparametric two-sample homogeneity test for matrices that we extend to the more general case of several groups. We first provide some theoretical results for the two associated test statistics and we explain how to derive change-point location estimators. Then, some numerical experiments are given in order to support our claims. Finally, our approach is applied to Hi-C data which are used in molecular biology for better understanding the influence of the chromosomal conformation on the cells functioning.

==> commande.tex <==
\newcommand{\1}{\mathbbm{1}}
\newcommand{\E}{\mathbb{E}}
\renewcommand{\P}{\mathbb{P}}


\newtheorem{Def}{Definition}

\newtheorem{rem}{Remark}

% Commands used by Sarah
\newcommand{\abf}{{\bf a}}
\newcommand{\alphabf}{\mbox{\mathversion{bold}{$\alpha$}}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Beta}{\mbox{B}}
\newcommand{\cbf}{{\bf c}}
\newcommand{\dd}{\mbox{d}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Dir}{\mbox{Dir}}
\newcommand{\Ibb}{\mathbb{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\mbf}{{\bf m}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\pibf}{\mbox{\mathversion{bold}{$\pi$}}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\thetabf}{\mbox{\mathversion{bold}{$\theta$}}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\Xbf}{{\bf X}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Ubf}{{\bf U}}
\newcommand{\Zbf}{{\bf Z}}


\newcommand{\proofbegin}{\paragraph{Proof.}}
\newcommand{\proofend}{$\blacksquare$\bigskip}
\newtheorem{thm}{Theorem}
\newtheorem{ex}{Example}
\newtheorem{prop}{Proposition}
\newtheorem{cor}{Corollary}
\newtheorem{lem}{Lemma}
\newtheorem{fact}{Fact}
\newtheorem{nota}{Notation}

\newcounter{hypA}
\newenvironment{hypA}{\refstepcounter{hypA}\begin{itemize}
  \item[({\bf A\arabic{hypA}})]}{\end{itemize}}

%% Lettres
\newcommand{\A}{A}
\newcommand{\bb}{b}
\newcommand{\B}{B}
\newcommand{\C}{C}
\newcommand{\D}{D}
\newcommand{\F}{F}
\newcommand{\f}{f}
\newcommand{\kk}{k}
\newcommand{\K}{K}
\newcommand{\lambdaa}{\lambda}
\newcommand{\Lambdaa}{\Lambda}
\newcommand{\el}{\ell}
\newcommand{\LL}{L}
\newcommand{\m}{m}
\newcommand{\M}{M}
\newcommand{\n}{n}
\newcommand{\PP}{P}
\newcommand{\tauu}{\tau}
\newcommand{\x}{x}
\newcommand{\X}{X}
\newcommand{\y}{y}
\newcommand{\Y}{Y}
\newcommand{\z}{z}
\newcommand{\Z}{Z}
\newcommand{\ii}{i}
\newcommand{\jj}{j}
\newcommand{\SSS}{S}
\newcommand{\ttt}{t}
\newcommand{\U}{{U}}
\newcommand{\aaa}{{a}}
\newcommand{\R}{R}
\newcommand{\h}{{h}}
\newcommand{\Sig}{\Sigma}

%% Variables
\newcommand{\bx}{{\bf \x}}
\newcommand{\bX}{{\bf \X}}
\newcommand{\xij}{\x_{\ii,\jj}}
\newcommand{\xji}{\x_{\jj,\ii}}
\newcommand{\Xij}{\X_{\ii,\jj}}
\newcommand{\Xipjp}{\X_{\ip,\jp}}
\newcommand{\Xijp}{\X_{\ii,\jp}}
\newcommand{\Xil}{\X_{\ii,\el}}
\newcommand{\Xiplp}{\X_{\ip,\lp}}
\newcommand{\Xilp}{\X_{\ii,\lp}}
\newcommand{\nun}{\n_{1}}
\newcommand{\Sn}{\SSS_{\n}}
\newcommand{\Uni}{\U_{\n,\ii}}
\newcommand{\Un}{\U_{\n}}
\newcommand{\Unun}{\U_{\n,1}}
\newcommand{\Unn}{\U_{\n,\n}}
\newcommand{\ai}{{\aaa_{\ii}}}
\newcommand{\bn}{{\bb_{\n}}}
\newcommand{\Unihat}{{\widehat{\Uni}}}
\newcommand{\Rni}{{\R_{\n,\ii}}}
\newcommand{\mcU}{{\mathcal{\U}}}
\newcommand{\mcR}{{\mathcal{\R}}}
\newcommand{\ip}{\ii'}
\newcommand{\lp}{\el'}
\newcommand{\aip}{{\aaa_{\ip}}}
\newcommand{\Unip}{{\U_{\n,\ip}}}
\newcommand{\Signun}{\Sig_{\n}\left(\nun\right)}
\newcommand{\bB}{{\bf \B}}
\newcommand{\bD}{{\bf \D}}
\newcommand{\lambdaun}{\lambdaa_1}
\newcommand{\lambdadeux}{\lambdaa_2}
\newcommand{\bM}{{\bf \M}}
\newcommand{\bA}{{\bf \A}}
\newcommand{\bC}{{\bf \C}}
\newcommand{\bP}{{\bf \PP}}
\newcommand{\tauun}{\tauu_{1}}
\newcommand{\dx}{\text{d\x}}
\newcommand{\dy}{\text{d\y}}
\newcommand{\dz}{\text{d\z}}
\newcommand{\dfx}{f(\x)\dx}
\newcommand{\dfy}{f(\y)\dy}
\newcommand{\dfz}{f(\z)\dz}
\newcommand{\hdeux}{\h_{2}}
\newcommand{\aiip}{\aaa_{\ii,\ip}}
\newcommand{\aii}{\aaa_{\ii,\ii}}
\newcommand{\Ln}{{\LL_{\n}}}
\newcommand{\Rn}{{\R_{\n}}}
\newcommand{\Xji}{\X_{\jj,\ii}}
\newcommand{\jp}{\jj'}
\newcommand{\ibis}{\zeta}
\newcommand{\ibisp}{\ibis'}
\newcommand{\Unibis}{\U_{\n,\ibis}}
\newcommand{\Unibisp}{\U_{\n,\ibisp}}
\newcommand{\aibisibisp}{\aaa_{\ibis,\ibisp}}
\newcommand{\aipip}{\aaa_{\ip,\ip}}
\newcommand{\aibispibis}{\aaa_{\ibisp,\ibis}}


%% Simplifications
\newcommand{\ligne}{{\cdot}}
\newcommand{\Xdotj}{{\X_{\ligne,\jj}}}
\newcommand{\Xdotun}{{\X_{\ligne,1}}}
\newcommand{\Xdotn}{{\X_{\ligne,\n}}}
\newcommand{\jzero}{{\jj_{0}}}
\newcommand{\jun}{{\jj_{1}}}
\newcommand{\Xijzero}{\X_{\ii,\jzero}}
\newcommand{\Xijun}{\X_{\ii,\jun}}
\newcommand{\hun}{{\h_{1}}}
\newcommand{\mcUn}{{\mcU_{\n}}}
\newcommand{\mcUnhat}{{\widehat{\mcUn}}}
\newcommand{\mcRn}{{\mcR_{\n}}}
\newcommand{\hzero}{{\h_{0}}}
\newcommand{\Xipjun}{{\X_{\ip,\jun}}}
\newcommand{\junp}{{\jj'_{1}}}
\newcommand{\Xipjunp}{{\X_{\ip,\junp}}}
\newcommand{\Xjuni}{{\X_{\ii,\jun}}}
\newcommand{\Xjzerojzero}{{\X_{\jzero,\jzero}}}
\newcommand{\ajzero}{\aaa_{\jzero}}
\newcommand{\ajun}{\aaa_{\jun}}
\newcommand{\Xjunjun}{{\X_{\jun,\jun}}}
\newcommand{\Xjunjzero}{{\X_{\jun,\jzero}}}
\newcommand{\Xjzerojun}{{\X_{\jzero,\jun}}}
\newcommand{\jzerop}{{\jj'_{0}}}
\newcommand{\Xipjzerop}{{\X_{\ip,\jzerop}}}
\newcommand{\Rkl}{\R_{\kk,\el}}
\newcommand{\Pkl}{\Prob_{\kk,\el}}
\newcommand{\Xijzerop}{{\X_{\ii,\jzerop}}}
\newcommand{\Xijunp}{{\X_{\ii,\junp}}}
\newcommand{\Signuniip}{\left[\Signun\right]_{\ii,\ip}}
\newcommand{\Signunii}{\left[\Signun\right]_{\ii,\ii}}
\newcommand{\Xiip}{{\X_{\ii,\ip}}}
\newcommand{\Xipi}{{\X_{\ip,\ii}}}
\newcommand{\unnunnun}{\mathds{1}_{\nun,\nun}}
\newcommand{\unnmnunnun}{\mathds{1}_{\n-\nun,\nun}}
\newcommand{\unnunnmnun}{\mathds{1}_{\nun,\n-\nun}}
\newcommand{\unnmnunnmnun}{\mathds{1}_{\n-\nun,\n-\nun}}
\newcommand{\Id}{\mathds{I}}
\newcommand{\unnn}{\mathds{1}_{\n,\n}}
\newcommand{\siminf}{\underset{+\infty}{\sim}}
\newcommand{\kzero}{\kk_{0}}
\newcommand{\kp}{\kk'}
\newcommand{\kzerop}{\kp_{0}}
\newcommand{\kun}{\kk_{1}}
\newcommand{\kunp}{\kp_{1}}
\newcommand{\Xikun}{{\X_{\ii,\kun}}}
\newcommand{\Xikunp}{{\X_{\ii,\kunp}}}
\newcommand{\Xikzero}{{\X_{\ii,\kzero}}}
\newcommand{\Xikzerop}{{\X_{\ii,\kzerop}}}
\newcommand{\Xipkun}{{\X_{\ip,\kun}}}
\newcommand{\Xipkunp}{{\X_{\ip,\kunp}}}
\newcommand{\Xipkzero}{{\X_{\ip,\kzero}}}
\newcommand{\Xipkzerop}{{\X_{\ip,\kzerop}}}
\newcommand{\Xibiskzero}{\X_{\ibis,\kzero}}
\newcommand{\Xibispkzerop}{\X_{\ibisp,\kzerop}}
\newcommand{\Xibiskun}{\X_{\ibis,\kun}}
\newcommand{\Xibispkunp}{\X_{\ibisp,\kunp}}
\newcommand{\Xjpip}{\X_{\jp,\ip}}
\newcommand{\Xjzeroi}{\X_{\jzero,\ii}}
\newcommand{\Xjzeropip}{\X_{\jzerop,\ip}}
\newcommand{\Xibisibisp}{\X_{\ibis,\ibisp}}
\newcommand{\Xibispibis}{\X_{\ibisp,\ibis}}
\newcommand{\Xiibis}{\X_{\ii,\ibis}}
\newcommand{\Xipibis}{\X_{\ip,\ibis}}
\newcommand{\Xiibisp}{\X_{\ii,\ibisp}}
\newcommand{\Xipibisp}{\X_{\ip,\ibisp}}

%% Notations usuelles
\newcommand{\mbR}{\mathbb{R}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Hzero}{\Hcal_{0}}
\newcommand{\Hun}{\Hcal_{1}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\var}{\mathbb{V}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\vrai}{\star}
\newcommand{\transpose}{^T}
\newcommand{\Esp}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\EspHzero}[1]{\mathbb{E}_{\Hzero}\left[#1\right]}
\newcommand{\tr}{tr}
\newcommand{\carac}{\mathcal{X}}
\newcommand{\mcB}{\mathcal{B}}
\newcommand{\mbN}{\mathbb{N}}
\newcommand{\mcN}{\mathcal{N}}
\newcommand{\mcC}{\mathcal{C}}
\newcommand{\mcE}{\mathcal{E}}

%% Notation pour la démo
\newcommand{\nuns}{\nun^{\vrai}}
\newcommand{\nunhat}{\widehat{\nun}}
\newcommand{\Pzero}{\Prob_{0}}
\newcommand{\Pun}{\Prob_{1}}

%%
\newcommand{\jzerobis}{{\jj''_{0}}}
\newcommand{\jzeropbis}{{\jj'''_{0}}}
\newcommand{\junbis}{{\jj''_{1}}}
\newcommand{\junpbis}{{\jj'''_{1}}}
\newcommand{\Xijzerobis}{{\X_{\ii,\jzerobis}}}
\newcommand{\Xijzeropbis}{{\X_{\ii,\jzeropbis}}}
\newcommand{\Xijunbis}{{\X_{\ii,\junbis}}}
\newcommand{\Xijunpbis}{{\X_{\ii,\junpbis}}}


%% Multiple
\newcommand{\nK}{\n_{\K}}
\newcommand{\nzero}{\n_{0}}
\newcommand{\Rij}{\R_{\ii,\jj}}
\newcommand{\Ripj}{\R_{\ip,\jj}}
\newcommand{\tbn}{{\bf \n}}
\newcommand{\bnK}{\tbn^{(\K)}}
\newcommand{\bR}{{\bf \R}}
\newcommand{\bRikK}{\bR_{\ii}^{(\kk)}\left(\bnK\right)}
\newcommand{\bRipkK}{\bR_{\ip}^{(\kk)}\left(\bnK\right)}
\newcommand{\bRunkK}{\bR_{1}^{(\kk)}\left(\bnK\right)}
\newcommand{\bRnkK}{\bR_{\n}^{(\kk)}\left(\bnK\right)}
\newcommand{\nk}{\n_{\kk}}
\newcommand{\nkun}{\n_{\kk+1}}
\newcommand{\bRkK}{\overline{\bR}^{(\kk)}\left(\bnK\right)}
\newcommand{\bS}{{\bf \SSS}}
\newcommand{\bSnK}{\bS_{\n}\left(\bnK\right)}
\newcommand{\bSig}{{\bf \Sig}}
\newcommand{\bSigkK}{\bSig_{\n}^{(\kk)}\left(\bnK\right)}
\newcommand{\bSigkKmoinsun}{\bSig_{\n}^{(\kk)}\left(\bnK\right)^{-1}}
\newcommand{\Ripjp}{\R_{\ip,\jp}}
\newcommand{\bSnKmax}{\bS_{\n,\K}^{(\text{max})}}


%% Algo Dyn
\newcommand{\tzero}{\ttt_{0}}
\newcommand{\tun}{\ttt_{1}}

%%%
\newcommand{\bm}{{\bf\m}}
\newcommand{\mcM}[2]{\mathcal{M}_{#1}\left(#2\right)}
\newcommand{\bi}{b_{\ii}}
\newcommand{\mnNzz}{\mathcal{N}_{\nun}^{00}}
\newcommand{\bbn}{{\bf\n}}
\newcommand{\mnNzu}{\mathcal{N}_{\nun}^{01}}
\newcommand{\mnNuu}{\mathcal{N}_{\nun}^{11}}
\newcommand{\mnN}{\mathcal{N}_{\nun}}
\newcommand{\Izz}{\mathcal{I}_{\nun}^{00}}
\newcommand{\Izu}{\mathcal{I}_{\nun}^{01}}
\newcommand{\Iuu}{\mathcal{I}_{\nun}^{11}}
\newcommand{\cizz}{c_{\jzero,\kzero}^{(i)}\left(\nun\right)}
\newcommand{\cizu}{c_{\lzero,\lun}^{(i)}\left(\nun\right)}
\newcommand{\ciuu}{c_{\jun,\kun}^{(i)}\left(\nun\right)}
\newcommand{\lzero}{\el_{0}}
\newcommand{\lun}{\el_{1}}
\newcommand{\Xilzero}{\X_{\ii,\lzero}}
\newcommand{\Xilun}{\X_{\ii,\lun}}
\newcommand{\mnNtot}{\mathcal{N}_{\nun}^{\text{tot}}}
\newcommand{\bbN}{{\bf N}}

%%% Hermite polynomials
\newcommand{\ccc}{c}
\newcommand{\p}{p}
\newcommand{\q}{q}
\newcommand{\pun}{\p_1}
\newcommand{\qun}{\q_1}
\newcommand{\pdeux}{\p_2}
\newcommand{\qdeux}{\q_2}
\newcommand{\HH}{H}
\newcommand{\functionc}[2]{\ccc_{#1,#2}}
\newcommand{\cpq}{\functionc{\p}{\q}}
\newcommand{\cqp}{\functionc{\q}{\p}}
\newcommand{\cpp}{\functionc{\p}{\p}}
\newcommand{\cpunqun}{\functionc{\pun}{\qun}}
\newcommand{\cqunpun}{\functionc{\qun}{\pun}}
\newcommand{\cpdeuxqdeux}{\functionc{\pdeux}{\qdeux}}
\newcommand{\cqdeuxpdeux}{\functionc{\qdeux}{\pdeux}}
\newcommand{\Hp}{\HH_{\p}}
\newcommand{\Hq}{\HH_{\q}}
\newcommand{\Hn}{\HH_{n}}
\newcommand{\Hpun}{\HH_{\pun}}
\newcommand{\Hqun}{\HH_{\qun}}
\newcommand{\Hpdeux}{\HH_{\pdeux}}
\newcommand{\Hqdeux}{\HH_{\qdeux}}
\newcommand{\Espphi}[1]{\mathbb{E}_{\phi}\left[#1\right]}
\newcommand{\SPQ}{\SSS_{n;P,Q}}
\newcommand{\hPQ}{\h_{P,Q}}
\newcommand{\gPQ}{g_{P,Q}}
\newcommand{\SnPQ}{\SSS_{\n,P,Q}}
\newcommand{\cpzero}{\functionc{\p}{0}}
\newcommand{\czeroq}{\functionc{0}{\q}}
\newcommand{\cpunzero}{\functionc{\pun}{0}}
\newcommand{\cpdeuxzero}{\functionc{\pdeux}{0}}
\newcommand{\czeroqun}{\functionc{0}{\qun}}
\newcommand{\czeroqdeux}{\functionc{0}{\qdeux}}


\newcommand{\muzero}{\mu_{(0)}}
\newcommand{\muMdeux}{\mu_{M_2}}

%%% Multiples ruptures
\newcommand{\LLL}{L}
\newcommand{\Ks}{\Ls}
\newcommand{\nKs}{\n_{\Ks}}
%\newcommand{\Ls}{\LLL^{\vrai}}
\newcommand{\Ls}{\LLL}
\newcommand{\nLs}{\n_{\Ls}}
\newcommand{\nL}{\n_{\LLL}}
\newcommand{\nLun}{\n_{\LLL+1}}
\newcommand{\SnunL}{\Sn\left(\nun,\ldots,\nL\right)}
\newcommand{\Rbar}{\overline{\R}}
\newcommand{\Rbarli}{\Rbar_{\el}^{(\ii)}}
\newcommand{\nl}{\n_{\el}}
\newcommand{\nlun}{\n_{\el+1}}
\newcommand{\Rji}{\R_{\jj}^{(\ii)}}
\newcommand{\Xik}{\X_{\ii,\kk}}
\newcommand{\Xikp}{\X_{\ii,\kp}}

\newcommand{\g}[2]{g\left(#1,#2\right)}
\newcommand{\Xiq}{\X_{\ii,\q}}
\newcommand{\Xip}{\X_{\ii,\p}}
\newcommand{\qp}{\q'}
\newcommand{\Xiqp}{\X_{\ii,\qp}}
\newcommand{\pp}{\p'}
\newcommand{\Xipp}{\X_{\ii,\pp}}




